Multi-Source Neural Variational Inference

Learning from multiple sources of information is an important problem in machine-learning research. The key challenges are learning representations and formulating inference methods that take into account the complementarity and redundancy of various information sources. In this paper we formulate a variational autoencoder based multi-source learning framework in which each encoder is conditioned on a different information source. This allows us to relate the sources via the shared latent variables by computing divergence measures between individual source's posterior approximations. We explore a variety of options to learn these encoders and to integrate the beliefs they compute into a consistent posterior approximation. We visualise learned beliefs on a toy dataset and evaluate our methods for learning shared representations and structured output prediction, showing trade-offs of learning separate encoders for each information source. Furthermore, we demonstrate how conflict detection and redundancy can increase robustness of inference in a multi-source setting.

==> sections/applications.tex <==
\section{Applications}\label{sec:applications}
% Robustness
% feature selection - if not too many, does not scale to too many
% distributed systems, data privacy
% anomaly detection. Note here that monolithic neural VI would eventually fail without user knowing
% lifelong learning
% cross-modal data generation

%As mentioned in section \ref{sec:introduction}, the integration of redundant or complementary information sources can lead to higher robustness and resolve ambiguities. 
%However, encapsulating the inferences into modules offers further advantages, compared to the integration within a monolithic neural network. 
%Next we present a selection of applications that may greatly benefit from modularity.
We have discussed methods to obtain modularized inference models, as well as compare and approximately integrate them. 
Such a form of modularization may be benefial for several different applications.
In the following, we briefly discuss a selected choice of applications.

\subsection{Multi-modal data generation}
In a system of modular inference models and likelihood functions, one can integrate sub-sets of information sources and generate likely data of other modalities, i.e.~infer missing data. 
Furthermore, if the LVM includes desired categorical data such as attributes or labels, one may infer latent representations from these attributes and generate random samples of the corresponding data type. 
We demonstrate this with class labels in Section \ref{sec:exp_multi_modal_generation}.

\subsection{Anomaly detection} \label{sec:anomaly_detection}
%As we gain access to the belief distribution of each information source's belief about the latent variables, we are able to compute useful divergence measures between them. 
%We can therefore not only calculated measures of redundancy, but even detect conflicting beliefs. 
%In the latter case, we should not integrate the beliefs. 
%Conflicting beliefs may stem from the data or an imperfect model. 
%The former is a form of data anomaly, while the latter signals that (parts of) the model cannot be trusted. 
%An imperfect model can be due to mis-specification or optimization problems and one may choose to re-train, remove or replace unreliable models. 

%Distinguishing between the two causes is requires evaluating the likelihood functions.
%Here we focus on data anomaly, assuming that the model fit the data reasonably well. 

% In the case of more than two information sources, the trust in one belief may be measured by the average KL divergence between one belief and all other beliefs.
% Here assume that the conflict is due to data anomaly.

Conflicting beliefs from different data sources---where the conflict stems from the data---is a form of data anomaly. 
A sensible measure for anomaly detection of this type can be obtained from Eq.~\ref{eq:conflict}.
We demonstrate the applicability of this measure in Section \ref{sec:exp_conflict_measure_anomaly}.
% Find the digits that have the highest conflict measure for un-modified digits. Will show digits whose parts are most surprising for each others source.
% Then apply random combinations of top and bottom digits within class and completely random. Same measure. 
% Evaluate the ranges of this measure to find a threshold to decide for anomaly and valid digit

\subsection{Distributed systems and data privacy}
Consider scenarios where different conditionally independent parts of observable data are distributed among multiple modules.
Suppose these this data either cannot or should not be communicated between modules.
This could be for computational reasons, communication bandwidth, or due to privacy concerns. 
Suppose further that associated information sources can be matched, i.e.~each module can retrieve its private samples based on unique shared keys.

In this scenario, we can learn individual modules without sharing raw data or the parameters of each module's inference and likelihood models.
For learning, we only need to share samples from the inference models as well as the likelihood values and gradients from the likelihood models w.r.t. the latent variable samples of each module. 
In order to integrate information, we need to share the inferred parameters of the variational distributions instead of the inferred latent variable samples.

The training procedure consists of the following steps:
Each module retrieves its private sample $\x_{m}$, based on a communicated key. 
Secondly, each module infers samples $\z_{m} \sim q_{\phi_{m}}(\z | \x_{m})$ and communicates these values to all other modules. 
The samples can be computed using the reparametrization trick \cite{KingmaW13}. 
In the third step, the likelihood functions $p_{\theta_{m}}(\x_{m} | \z_{m'})$ are evaluated for the latent variable samples $z_{m}$ of the same module, as well as the samples $z_{m'}$ received from other modules.
The gradients are evaluated w.r.t. all latent samples. The gradients and likelihood values are then communicated back to the corresponding modules $m'$. 
%The parameters of the likelihood functions can now be updated. 
Lastly, each module calculates the gradients for its inference models, continuing back-propagation from the communicated and its own gradients. 
With $K > 1$, the gradients need to be weighted by the average importance weights, which can be calculated from the communicated likelihood values \cite{BurdaGS15}.
%
%Post training, any subset of modules in this distributed system may be integrated.
%
\newline
We note that all of the experiments in section \ref{sec:experiments} could be implemented in this distributed form. 
% In some experiments however, we chose to share some parameters of all likelihood functions for simplicity. 
%%% \TODO{Make instead just all experiments with modular NN. }
% We show the equivalence between multiple or a single neural network experimentally, based on log-likelihood scores on our modified partially observable modifications of mnist. 

\subsection{Life-long learning}
%
%\newline
%%
%We conjecture that modularity is particular important if we want to move current deep learning methods towards lifelong learning (LLL) systems \cite{SSS135802}. 
%Some of the key challenges of this learning paradigm can be greatly facilitated in a modular system.
%Consider a system where modules can be evaluated both individually and jointly and even compared to each other. 
%Decisions for selective knowledge retention, erasure or transfer, can then be made based on performance and divergence measures of and between the modules. 
%\TODO{Still not good. Consider removing LLL from introduction anyway. Maybe only in application.}

%This learning paradigm has several challenges such as continual learning, knowledge retention and transfer, and reusing previously acquired knowledge to facilitate further learning \cite{SSS135802}. 
%%Another problem in this field is to deal with conflicting information.
%These problems may be greatly facilitated in modular systems. 
%Redundant, unreliable or conflicting modules may be removed or replaced and already trained modules can facilitate learning of new modules.

%In life-long machine learning, agents are required to learn one or more tasks continually and eventually adapt to changing data distributions. 
%At the same time the agent should not forget previously learned tasks that might be required in the future. 
Life-long machine learning is a paradigm in which agents are required to learn multiple tasks continually \cite{SSS135802}. 
This paradigm poses many challenges, such as selective knowledge retention, erasure or transfer between tasks. 
Furthermore, previously learned tasks or acquired knowledge should be used to improve further learning.
\newline
Some of these challenges can be tackled in our modular neural variational inference framework. 
For example, redundancy of whole modules can be quantified using the expected value of the measure defined in Eq.~\ref{eq:redundancy}, where the expectation is over samples in the dataset.
In the case of high redundancy, the module could be removed to free up computational resources. 
\newline
Furthermore, modules being in conflict with all others can be detected during life-time using the measure from Eq.~\ref{eq:conflict}. 
Depending on the cause of conflict, unreliable modules may be retrained, removed or replaced. 


Retraining or training new modules during the system's life time can also benefit from already trained modules. 
To re-train or integrate $L$ new modules into the existing system, one can maximize the objective $\elboa$ with the sum over information sources instead counting from $m=M$ to $M+L$. 
Note that this objective requires the evaluation of all likelihood functions though, in order to ensure a coherent latent space. 
However, reusing the existing likelihood functions can speed up learning of the new modules. 
\newline
If the new source is complementary rather than redundant, the existing latent representation could be altered by adding additional latent variables.
Alternatively, a Bayesian treatment of the model parameters allows for small adaptations of the existing likelihood function to the new modules \cite{NguyenV, Kirkpatrick3521}. 











